Are LLM Agents Behaviorally Coherent? A Latent Profiling Approach for Social Simulation

LLM agents are increasingly proposed as substitutes for human participants in social research, usually on the strength of survey responses that match those of the humans they represent. We argue that such output-level alignment is not enough. Drawing on the behavioral sciences, we propose Latent Profiling, a framework for testing behavioral coherence: whether an agent's conversational behavior follows, as human behavioral models predict, from its own latent profile elicited by short surveys. As a case study, we test six hypotheses about preference, openness and agreement across nine open models. Agents reproduce surface-level trends but systematically fail in-depth tests: they are not behaviorally coherent, even when their individual responses look human. Latent Profiling thus offers a theory-grounded instrument for a behavioral science of LLMs.

==> acl_lineno_fix.tex <==
\makeatletter
\@ifpackageloaded{lineno}{%
  \@ifpackagelater{lineno}{2026/02/01}{%
    \IfFormatAtLeastTF{2026-06-01}{}{%
      \RemoveFromHook{build/column/before}[lineno]%
      \AddToHook{begindocument/end}{%
        \def\@LN@makecol{%
          \@LN@orig@makecol
          \setbox\@outputbox\vbox{%
            \boxmaxdepth\@maxdepth
            \protected@write\@auxout{}{%
              \string\def\string\@LN@column{\if@firstcolumn1\else2\fi}}%
            \box\@outputbox}}}%
    }%
  }{}%
}{}
\makeatother

